Sampling from Discrete Energy-Based Models with Quality/Efficiency Trade-offs

Energy-Based Models (EBMs) allow for extremely flexible specifications of probability distributions. However, they do not provide a mechanism for obtaining exact samples from these distributions. Monte Carlo techniques can aid us in obtaining samples if some proposal distribution that we can easily sample from is available. For instance, rejection sampling can provide exact samples but is often difficult or impossible to apply due to the need to find a proposal distribution that upper-bounds the target distribution everywhere. Approximate Markov chain Monte Carlo sampling techniques like Metropolis-Hastings are usually easier to design, exploiting a local proposal distribution that performs local edits on an evolving sample. However, these techniques can be inefficient due to the local nature of the proposal distribution and do not provide an estimate of the quality of their samples. In this work, we propose a new approximate sampling technique, Quasi Rejection Sampling (QRS), that allows for a trade-off between sampling efficiency and sampling quality, while providing explicit convergence bounds and diagnostics. QRS capitalizes on the availability of high-quality global proposal distributions obtained from deep learning models. We demonstrate the effectiveness of QRS sampling for discrete EBMs over text for the tasks of controlled text generation with distributional constraints and paraphrase generation. We show that we can sample from such EBMs with arbitrary precision at the cost of sampling efficiency.

==> sections/OLDS/intro_orig.tex <==
\annot{Can't sample from EBMSs} In Machine Learning problems, it is often important to be be able to obtain samples from a generative model defining a probability distribution $p(x)$ over elements in a sampling space $X$. In many cases, when this probability distribution is provided in normalized form, this can be easily done.
For example, auto-regressive sequence models factorize the probability of a sequence as a product of token-level probabilities.
Then, sampling sequences reduces to sampling one token at a time.
However, this simplicity in sampling comes at the cost of considerable difficulty in incorporating sequence-level functions in the computation of probability scores.
Energy-Based Models (EBMs)~\citep{lecun_tutorial_2006} enjoy a greater representational freedom by mapping elements into arbitrary unnormalized non-negative scores $P(x)$.
In particular, EBMs over sequences (Sequential EBMs) have been leveraged by prior studies to tackle many different tasks, including Controlled Natural Language Generation~\citep{khalifa_2021}, Natural Language Understanding~\citep{he-etal-2021-joint}, Language Modelling~\citep{Deng_EBM_20}, Machine Translation~\citep{Naskar2020EnergyBasedRI}, and data-efficient learning~\citep{A-parshakova-etal-2019-global}.
However, what is gained in expressive power is also lost in the ability to sample from the probability distribution associated with the EBM.%, namely $p(x) = P(x)/Z$, where $Z=\sum_{x \in X}{P(x)}$ is the partition function, and $X$ is the sampling space.

\annot{Fine-tuning problems} One possibility for obtaining samples, exploited by \citet{khalifa_2021} in the context of Controlled Text Generation, is to fine-tune an autoregressive policy $\pi_\theta(x)$ that approximates the probability $p(x) = P(x)/Z$ induced by the EBM, where $Z=\sum_{x \in X}{P(x)}$ is the partition function.
This policy has the advantage that now it is possible to sample from it.
However, this approach suffers from some drawbacks.
Firstly, it might be very hard or impossible, in practice, to approximate the target EBM to an arbitrary precision.
For instance, the authors define an EBM that controls the distribution of a language model to only generate biographies of scientists, while also imposing that 50\% of them should mention females.
However, the sentences actually generated by the autoregressive policy are only talking about scientists in 70\% of the cases, and in only 30\% of the cases mentioning a female character.
Moreover, theoretical limitations of autoregressive models may prevent them from ever being able to express the function represented by the EBM~\citep{LinJLGE21}. 

In fact, it can sometimes be impractical to fine-tune a policy for certain tasks. 
Consider, for instance, the problem of removing toxic sequences from a language model where these sequences are already rare (e.g., only $0.01$\% are toxic). 
This problem can be readily tackled by simply filtering out toxic sequences from the samples, instead of fine-tuning the model to exclude the sequences.
Note also that, in standard autoregressive architectures, it can be theoretically impossible to fine-tune a model to completely exclude a certain kind of sequences, because a softmax-based language model will always assign some probability mass to them.\fmd{(23/08/2021) I feel this important paragraph needs more work. Not sure exactly how, perhaps: better separate the theoretical observations from the practical ones, simplify the practical example to just a simple condition (amazing), document the theoretical issues more...}


%With the advent of large Language Models (LMs), it is relatively easy to generate high-quality natural language utterances by autoregressively sampling token sequences.
%Yet, sampling directly from these models will reproduce the statistics found in the training corpora, which may not always be desirable as it can reproduce biases\citep{??}, exhibit toxicity\citep{??} or other unwanted behaviours\citep{??}.
%Thus, the problem of \emph{controlling} what kind of content goes into these sentences has become increasingly important.


\annot{Monte-Carlo techniques} Even if imperfect, we note that having a good approximation from which we can sample can constitute a powerful ally if used as a proposal distribution $q(x)$ for the appropriate Monte-Carlo (MC) technique.
One simple possibility would be to apply Rejection Sampling (RS).
However, standard RS suffers from an important drawback, namely, the practitioner must know the value of a finite upper-bound $\beta$, satisfied by all $x \in X$, on the score ratio $P(x)/q(x)$ between the unnormalized target distribution $P$ and the proposal distribution $q$.
However, it is often hard or impossible to find such a bound.
Moreover, even if a bound can be found but is large, then the method can be extremely inefficient, as is the typical case in  high-dimensional spaces \citep{andrieu2003introduction}.
In such cases, Markov Chain Monte-Carlo (MCMC) techniques are often preferred ~\citep{RJ_casella2004generalized,robertMetropolisHastingsAlgorithm2016}, with the Metropolis-Hastings algorithm~\citep{metropolis1953equation,hastings1970monte} a popular choice.
One advantage of these methods is that even if we cannot find a good \emph{global} proposal (i.e., a proposal that can produce reasonable samples from all the sample space), we can still use \emph{local} transitions in the sample space~\citep{rosenthalOptimalProposalDistributions2011,zanellaInformedProposalsLocal2017}, which can be easier to formulate. However, the disadvantage of local transitions is that the sampler can easily get trapped into portions of the space from which it cannot easily escape, therefore preventing it to explore all the relevant parts of the space. 

\annot{QRS} In this paper, we introduce Quasi Rejection Sampling (QRS), an MC technique that generalizes Rejection Sampling (RS) and allows a controllable trade-off between the approximation quality of the sampler and its efficiency.
Unlike RS, QRS does not require using an absolute $\beta$ upper-bound, or even that such a bound exists at all.
Instead, it interprets $\beta$ as a threshold that upper-bounds $P(x)/q(x)$ for only a portion of the sample space. 
Informally, the intuition is that if we can find a $\beta$ that bounds the ratio for not all but a large part of the $p$-mass of $X$, then this part of the sample space can be recovered precisely, while the rest can be approximated with some error.\fgk{correct? \textcolor{blue}{MD: a bit imprecise, but gives the main intuition, I think.}}
%Formally, we demonstrate that the TVD between the distribution of the sampler at any chosen $\beta$ and the target distribution is bounded by $1-p\left(\{x \in X : P(x)/q(x)\right \leq \beta\})$.
\fmd{I propose to leave out for now this paragraph: \textit{We also note that, in contrast to the time when MCMC techniques were first proposed, such high-quality global proposal distributions are now available even for very complex high-dimensional spaces thanks to neural network models.}. I have tried to reformulate it a bit but I am struggling to find the right place for it now... Let's go back to it later.}
QRS formalizes these intuitions as explicit convergence bounds, while also providing precise estimates of the sampling quality (i.e., the distance of the sampling distribution to the target distribution) and efficiency (i.e., the sampler's acceptance rate).
%\gk{@Marc, please have a look at how to best formulate this sentence}, 
Crucially, these diagnostics are typically \emph{not} available in MCMC algorithms such as Metropolis-Hastings.

\annot{Samples vs. Expectations + Main idea of QRS} We focus on the task of obtaining \emph{samples} from an unnormalized model for the purpose of using these samples in some downstream application. This is different from the typical use of many samplers like MCMC, where often the primary goal is to estimate the \emph{expectation} of some function. 
%
%In such cases one can use independent Metropolis-Hastings (IMH) or importance sampling (IS) in combination with some unconditional, global, proposal distribution in order to estimate such expectations, or in case such a global proposal is not available one can use some local, conditional, proposal distributions or posteriors for random walk Metropolis-Hastings or Gibbs sampling. The Markov chain central limit theorem~\citep{Robert:2004} guarantees that the estimate of these expectations converges to the true value.%
%
In order to estimate such expectations, one can use Importance Sampling (IS) in combination with some unconditional, global, proposal distribution, or in case such a global proposal is not available one can use some local, conditional, proposal distributions or posteriors for random walk Metropolis-Hastings or Gibbs sampling. The Convergence Theorem for Metropolis-Hastings Markov Chains ~\citep[Theorem 7.4.(i) p. 274]{Robert:2004} guarantees that the estimate of these expectations converges to the true value for chains of increasing length.\footnote{However it does not provide a concrete procedure for assessing the convergence speed.} \fmd{(31-08-2021) I have taken the liberty to edit a bit the original text (commented in the source) to de-stress IMH for computing expectations (assuming it under general MH) and also to be more precise in which convergence theorem is actually needed from Robert-Casella. My impression is that the various "Central Limit" theorems from this text are not the most relevant ones here.}
%
One downside of any of the MH-type algorithms for obtaining samples for use directly in some downstream application, rather than estimating expectations, is the high autocorrelation among samples, or even many repetitions (also see Appendix~\ref{sec:app:qrs_vs_imh}).
If a good global proposal distribution is available and we can find some reasonable  constant with which we can bound the unnormalized distribution we wish to sample from, we can use rejection sampling to obtain exact samples from the target distribution. We extend this approach by providing the possibility to \textit{approximately} sample from the target distribution even when we cannot find such a bound. Obtaining samples can be useful for many applications, e.g. debiasing a language model~\citep{khalifa_2021}, obtaining a diverse set of outputs~\citep{holtzman-etal-curious-2020}\fbe{This is maybe not the best citation, can anyone think of a better one?} or as inputs to some decision rule~\citep{eikema-aziz-sampling-2021}.\fmd{(01-09-2021) Another possible application would be to obtain a large ``virtual'' dataset of samples from an EBM, from which an autoregressive policy could be obtained by standard supervised learning; this either as an alternative or as a complement to DPG.}

\annot{Evaluation task}To show the effectiveness of \QRS, we experiment with Controlled Text Generation,
partially following the setting of \cite{khalifa_2021}. 
The goal here is to adapt the distribution of a pretrained language model over sequences $x$ to make the expectations (aka moments) of some features of $x$ match some desired values (e.g., 100\% of the sequences must refer to science and 50\% to females), while remaining as close as possible to the pretrained model. 
\cite{khalifa_2021} show that these requirements naturally result in a certain EBM formulation. 
The remaining question is how to actually obtain samples from this EBM.
%
\annot{Proposals} To this end, we explore two alternatives, both based on QRS, but exploiting two different kinds of proposal $q$.
The first one takes as proposal the fine-tuned distribution obtained in \citet{khalifa_2021}, which 
approaches the target EBM, but still can leave a large gap as mentioned previously. 
%
The second one uses \emph{prompts} to condition a pre-trained language model~\citep{Brown2020LanguageMA}.
While prompts have been studied extensively to obtain samples for many different purposes~\citep{Brown2020LanguageMA,petroni2019language,qinLearningHowAsk2021,liPrefixTuningOptimizingContinuous2021}, the exact properties of these samples cannot be precisely controlled.
Here, we suggest that these imprecise distributions can instead make good proposals for obtaining \emph{unbiased} samples from a target EBM with precisely controlled properties. 
%
\annot{Results}Our results show that we can approximate the target distribution to any arbitrary level of accuracy
if we are willing to pay a higher cost in terms of sampling efficiency. The trade-off between these two conflicting objectives can be computed explicitly within QRS, allowing user-defined choices depending on the intended applications of the algorithm.
%
\fmd{(23-08-2021) global note: wondering whether it would be good to add in the Appendix some notes on the practical differences between a non-scoring sampler and a scoring sampler, for instance why we can estimate $KL(p_\beta,a)$ but not $KL(imh,a)$ for instance. Things that otherwise are only implicit in the plots.}

==> sections/related_work_old.tex <==

Sampling from EBMs does not necessarily %need access to a proposal distribution. 
\ptmd{need to take a Monte Carlo approach.}\fmd{(01-10) DPG does also need a proposal distribution...}
As noted above, DPG~\citep{opt-rl-arxiv-2019} allows to train an autoregressive model that approximates an arbitrary EBM, which can then be used to sample. However, it might be very hard or impossible, in practice, to approximate the target EBM to an arbitrary precision because of the complexity of the EBM, or even more seriously, because of theoretical limitations of autoregressive models~\citep{LinJLGE21}.
%Taken from previous discussion (don't feel this is the right place to elaborate on this):
%For instance, while the authors define an EBM that controls the distribution of a language model to generate biographies of scientists, 50\% of which should be female, the sentences generated by the autoregressive policy are only talking about scientists in 70\% of the cases, and in only 30\% of the cases mentioning a female person.
%Moreover, theoretical limitations of autoregressive models may prevent them from ever being able to express the function represented by the EBM~\citep{LinJLGE21}. 
%Furthermore, it can sometimes be impractical to finetune a policy for certain tasks. 
%Consider, for instance, the problem of removing toxic sequences from a language model where these sequences are already rare (e.g., only $0.01$\% are toxic). 
%This problem can be readily tackled by simply filtering out toxic sequences from the samples, instead of fine-tuning the model to exclude the sequences, which can also be theoretically impossible to achieve in standard autoregressive architectures, because a softmax-based language model will always assign some probability mass to them.


Here we have proposed an extension of Rejection Sampling. Many variations of rejection sampling (also going under the name of ``Accept-Reject'')  techniques have been studied in the past~\citep{martino2018accept}.
Perhaps the one least related to our approach is the Sampling Importance Resampling (SIR) algorithm~\citep{rubin1987calculation, skare2003improved} which prescribes to obtain a candidate set of samples from the proposal distribution, and then re-sample from these samples according to the importance ratios. While we do not compare to this approach, there are obvious drawbacks to it. For instance, all elements not included in the candidate set will be given 0 probability, and SIR provides no diagnostics of the approximation quality.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
More similar to the here described technique, \citet{caffo2002empirical} propose Empirical Supremum Rejection Sampling (ESRS), an algorithm that iteratively adapts the $\beta$ upper-bound. 
While QRS can use such adaptive schemes (see Appendix \ref{appx:qrs_extensions}), it can also be applied to a fixed $\beta$ parameter.
More importantly, ESRS requires that there exists a finite $\beta$ --- perhaps unknown --- that upper-bounds $P(x)/q(x)$ for all $x$, whereas this is not required by QRS (viz. Section \ref{sec:poisson}).
Others have observed before that a generic $\beta$ parameter that does not upper-bound the full space leads to the probability distribution in Eq. \ref{eq:p_beta}~\citep{ Robert:2004,martino2018accept}.\fmd{(01-09-2021) I think we should be more precise in terms of equations or pages in book-length references, otherwise it is difficult and sometimes ambiguous what we exactly refer to. We can use the form \texttt{\textbackslash cite[p.~PPPP]\{XXXX\}} for that.}
In particular, two strategies have been proposed that make use of this observation.
% The first is Rejection Sampling Chains~\citep{tierney1992exploring}\fmd{See also \citep[\S 6.1]{chib1995understanding}} and Adaptive Rejection Metropolis Sampling~\citep{gilks1995adaptive}; \citep[\S 2.4.2]{Robert:2004} in which this definition is combined with IMH to produce a Markov Chain that converges to the correct stationary distribution.
The first is Rejection Sampling Chains~\citep{tierney1992exploring}, \citep[\S 6.1]{chib1995understanding} in which this definition is combined with IMH to produce a Markov Chain that converges to the correct stationary distribution.
The second is Rejection Control (RC)~\citep{liu1998rejection}, which sub-samples a set of samples using a procedure akin to QRS, and then uses these samples to obtain unbiased IS estimates of quantities of interest.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Closer to our technique, \citet{caffo2002empirical} propose Empirical Supremum Rejection Sampling (ESRS), an algorithm that iteratively adapts the $\beta$ upper-bound. 
While QRS can use such adaptive schemes (see Appendix \ref{appx:qrs_extensions}), it can also be applied to an arbitrary $\beta$ parameter.
Importantly, while ESRS requires that there exists such a $\beta$ --- perhaps unknown --- that upper-bounds $P(x)/q(x)$ for all $x$, this is not required by QRS\ifnotworkshop(cf. Section \ref{sec:poisson})\fi.
%
Some other techniques do not require a global upper bound. Rejection Sampling Chains~\citep{tierney1992exploring}, \citep[\S 6.1]{chib1995understanding} 
use rejection sampling in a region satisfying a partial upper-bound but combine it with IMH outside of that region to produce a Markov Chain that converges to the correct stationary distribution in the limit.
Still others have observed before us that a generic $\beta$ parameter that does not upper-bound the full space leads to the probability distribution presented in Eq. \ref{eq:p_beta}. In particular Rejection Control (RC)~\citep{liu1998rejection}, \citep[pp. 44-45]{liu2004Book} makes use of this observation for accelerating the computation of an unbiased IS estimate of the expectation $\E_{x\sim p}f(x)$ for situations in which computing $f(x)$ is expensive and where it is desired to reduce such computation in regions of $p$ for which the importance ratios are small and have less impact on the IS estimate.
%
To the best of our knowledge, all of these techniques have focused on estimating expectations $\E_{x\sim p}f(x)$, whereas here we study how to obtain individual samples from the target distribution $p$ that can be used for specific applications, such as debiasing language models.
The proposed approach relaxes the constraint of obtaining a sampler perfectly matching the target EBM --- an objective that is often only attainable in the theoretical limit --- in favour of a more flexible technique that allows to trade-off quality with efficiency.
Furthermore, we give explicit diagnostics to inform this trade-off, namely, an upper bound on the TVD between the sampler and the target distribution (viz. Eq. \ref{eq:qrs_upper_bound})  and an unbiased estimate of this distance (Eq. \ref{eq:qrs_tvd}).
%%%%%%%%%%%%%%%%%%%
% \fmd{(01-09-2021) (Some comments on my editions about this part of the related work --- for discussion)\\
% I removed the reference to Gilks (ARMS) as I did not see such a clear connection with our equation \ref{eq:p_beta} and also because the focus on log-concavity appears to me to be aimed at 1-dim real spaces $X$, very different from our space. Overall, not convinced of the relevance of this reference.\\
% On the other hand, the reference to Liu (I looked only at his book) appears very relevant, and I hope that what I say in the text is correct (look in particular at the paragraph on top of his page 44 about his motivation). His equation (2.15) is the same as our equation (1) but he exploits it for different purposes than ours. However, if we look at his theorem (2.6.1), I think he could have exploited it for observing that with increasing $\beta$, the chi-square ``distance'' between $p$ and $p_\beta$ (in our notation) decreases. This pseudo-distance (not symmetrical) could then probably be exploited for a similar trade-off to what we have with TVD. But Liu's focus was on expectations, not on sampling. Still, not so far from us. Food for thought for our ICLR version?}
%%%%%%%%%%%%%%%%%%%

%Several works used constraints beam search~\cite{AndersonFJG17,hokamp-liu-2017-lexically,PostV18} as a way of lexically constrained decoding from pretrained models. Compared to our method these methods have the following drawbacks: they can only handle "lexical" pointwise constraints, as well as their reliance on beam search makes it impossible to sample from the pre-trained model in an unbiased way.\fbe{I don't believe this paragraph to be that related to our current work.}   
